Finding Temporally Consistent Occlusion Boundaries in Videos using Geometric Context

We present an algorithm for finding temporally consistent occlusion boundaries in videos to support segmentation of dynamic scenes. We learn occlusion boundaries in a pairwise Markov random field (MRF) framework. We first estimate the probability of an spatio-temporal edge being an occlusion boundary by using appearance, flow, and geometric features. Next, we enforce occlusion boundary continuity in a MRF model by learning pairwise occlusion probabilities using a random forest. Then, we temporally smooth boundaries to remove temporal inconsistencies in occlusion boundary estimation. Our proposed framework provides an efficient approach for finding temporally consistent occlusion boundaries in video by utilizing causality, redundancy in videos, and semantic layout of the scene. We have developed a dataset with fully annotated ground-truth occlusion boundaries of over 30 videos ($5000 frames). This dataset is used to evaluate temporal occlusion boundaries and provides a much needed baseline for future studies. We perform experiments to demonstrate the role of scene layout, and temporal information for occlusion reasoning in dynamic scenes.

==> classification.tex <==
\subsection{Classification}
\label{sec:classification}

We use a random forest classifier to estimate the occlusion probability of an edgelet. Random forest provide feature selection, and good estimate of feature importance~\cite{breiman2001random,saeys2008robust}. We trained random forest with 105 trees, 11 random features per node, and a maximum depth of 35 nodes for a tree. We train the classifier with the features listed in \Cref{Table:feat_occl} from each edgelet of each frame to capture the temporal variations.
 
To predict occlusion boundaries for a test video, we compute occlusion features for each edge of each frame in the over-segmented video. Then a random forest assigns each edgelet a probability for being occlusion boundary.  Now, we have assigned each edgelet an occlusion probability and thresholding these probabilities would give occlusion boundaries. However, these estimates are not temporally consistent, \textit{i.e.}, occlusion probability of an edgelet can change significantly from one frame to next. To provide temporal consistent occlusion boundaries, we leverage from video segmentation to temporally smooth the occlusion probability of an edge over a temporal window. We experiment with different lengths of temporal windows to filter out temporally inconsistent boundaries (\Cref{sec:results}). 

%Next, we enforce geometric consistency explicitly by providing the geometric potential to the CRF model. The CRF models aims at improving the occlusion boundary detection by suppressing occlusion boundaries found in sky, and ground region, and penalizing absence of occlusion boundary between different geometric classes.
%To train a pairwise classifier, we compute the pairwise features by concatenating the unary features, and adding the continuity features. The positive pairwise edge examples are the edges with ground truth label "ON", and the negative examples are the one where an edge with ground truth label "OFF" is followed by an edge labelled "ON". We evaluate our method over 5-fold cross-validation.

%To predict occlusion boundaries for a test video, we compute unary and pairwise features for each edge of each frame in the over-segmented video. We estimate the final probability of an edge being "ON" by providing the surface, and junction potential using the CRF model. This gives a probability estimate for each edge being "ON" or "OFF". However, these estimates are not temporally consistent, i.e., probability of an edge label can change significantly from one frame to next. To provide temporal consistent occlusion boundaries, we leverage from video segmentation to temporally smooth the occlusion probability of an edge over a temporal window ,e.g., 30 frames from the first appearance of the edge.  


==> crf.tex <==
\subsection{CRF Model}
\label{sec:crf}

Using the broad range of features described earlier, we can classify each edgelet as being "ON" (on occlusion boundary) or "OFF" (not on occlusion bounday). However, to enforce global reasoning, and enforce continuity and geometric consistency we use a conditional random field (CRF) model. Our goal is to maximize the probability of an edgelet being "ON" given feature vector x, $P(e|data)$. We can estimate this probability by factor graph, where a factor corresponds to,

$P(e|data)\propto \Pi_i\psi_i \Pi_j\phi_j$,

\noindent where, $\psi_i$ and $\phi_j$ are the surface and junction factors. This CRF model performs joint inference over surface, and boundary estimates, enforcing boundary continuity and geometric consistency. Boundary factors encode the likelihood for an edgelet being "ON" given the its feature vector $x$ and the probability of the preceding edgelet $P(e_i|e_{i-1},x)$. Surface factors encode likelihood of edgelet label given the feature vector $x$ and surface confidence. Surface factors encode geometric consistency by imposing a penalty for lack of boundary between different geometric classes, and for occlusion boundaries within sky, and ground region. The exact solution of the inference is intractable. We obtain the approximate solution by combining Heskes \etal\cite{} with Yuille~\etal\cite{} mean-field approximation \cite{Hoeim, Stein}. \hrnote{I want to compute that from depth-ordered layers, which I dont have yet :(}
%Our CRF model is similar to previously proposed models \cite{Hoeim, Stein} but we do not include figure/ground labels. 









==> discussion.tex <==
%\section{Discussion}
%\label{label:discussion}
%Our goal in this paper is to find temporally consistent occlusion boundaries. We achieve this by leveraging spatio-temporal video segmentation, and scene layout in a pairwise edge continuity MRF framework. The results shown above are computed on the spatio-temporal boundaries provided by video over-segmentation \cite{MatthiasSegmentation}. We choose graph-base video segmentation algorithm for its accuracy, temporal coherence, and ability to handle long video sequences efficiently. Our approach for learning occlusion boundaries is independent of any particular video segmentation algorithm and should perform well using other video over-segmentation algorithms. 


%In addition, we propose to efficiently process videos by exploiting temporal redundancy and causality with temporal smoothing. 


==> experiments.tex <==
\section{Experiments}
\label{sec:experiments}



==> occl_vidseg.tex <==
\section{Occlusion-aware Video Segmentation}
\label{sec:occl_vidseg}
%%% intor , y occlusion-aware segmentation, temporally consistent, usefulnes, applications, how, n resutls

%%%intro, y occl seg
A fundamental challenge is to extract spatio-temporal boundaries or regions of objects and their semantic classes in videos. A solution to this problem can benefit a broad range of problems, \textit{e.g}, object detection, recognition, tracking, and feature extraction. Typically, this goal is achieved by grouping together regions that are similar in color and visual features, without accounting for occlusions. This results in a large number of regions and boundaries for individual objects or classes. In contrast, occlusion-awareness can provide strong features to improve object segmentation by removing weak, non-occlusion boundaries while preserving strong color and occlusion boundaries. To achieve this occlusion-awareness, we propose an extension to the video segmentation algorithm of Grundmann~\etal\cite{MatthiasSegmentation}. Grundmann \etal \cite{MatthiasSegmentation}, proposed an efficient graph-based video segmentation algorithm, which constructs a graph across video frames grouping pixels which exhibit similarity in appearance and motion. First pixels in the video volume  are grouped together based on color similarity, then for each resulting region descriptors in form of \textit{L*a*b*} histograms and optical flow histograms are computed, providing a richer appearance and motion description. These regions are then further grouped based on the $\chi^2$-difference of their descriptors resulting in a hierarchy of super-regions.
We improve upon on their graph construction, by including the occlusion probabilities as a weighted term for estimating the similarity between pixels. For instance, when comparing two pixels $x_i$, $x_j$ the cost on their edge is
\begin{align} \label{eq:occl_wt}
d(x_i,x_j) \,=\,\,& (1-w_{\mathcal{O}})\|L(x_i) - L(x_j)\|_2 \,\, + \notag \\
& w_{\mathcal{O}}\left|\mathcal{O}(x_i) - \mathcal{O}(x_j)\right|,
\end{align}
where $w_{\mathcal{O}}$ is the occlusion weight, $L(\cdot)$ is the \textit{L*a*b*} color, and $\mathcal{O}(\cdot)$ are the probabilities computed by the occlusion boundary classifier. By adding occlusion probabilities we force boundaries at pixels with high occlusion probabilities, and merge regions separated by low probable occlusion boundaries. Based on these edge weights , a 3D space-time graph is constructed, giving spatio-temporal regions that are coherent in color, and occlusion. Note that our goal here is to develop a method to group regions that are temporally consistent in both appearance and occlusion as opposed to occlusion alone. \Cref{fig:occl_seg} compares the appearance only based video segmentation of \cite{MatthiasSegmentation}, with our occlusion-aware segmentation at the over-segmentation stage.

\begin{figure*}[ht]
\centering
\vspace{-0.5cm}
\includegraphics[width=0.85\textwidth]{fig_vid_occl2.pdf}

\caption{\small{Comparison of color based video segmentation with color+occlusion based video segmentation. Occlusion-aware video over-segmentation prevents spurious boundaries between regions separated by weak occlusion boundaries, but preserves boundaries with stronger color and occlusion probabilities, given by \Cref{eq:occl_wt}. The results in the above figure are generated by setting $w_{\mathcal{O}}$ to $0$ for color, and $0.25$ for occlusion-aware segmentation, respectively.}}

\label{fig:occl_seg}
\end{figure*}



%%% purpose is not to give only occlusion boundaries but a balance of occlusion n appearance regions ;)

%spatio-temporal regions over an over-segmented video volume. The video segmentation algorithm first segments

%Their video segmentation algorithm co 3d space-time graph over image segmentation proposed by Felzenszwalb\etal\cite{}.  

%We now revisit the video segmentation and propose an extension by adding occlusion-awareness. 



%%% example, figure, gt(red occl boundaries, black non-occl boundaries) , prediction

==> occlusion_data.tex <==
\section{Dataset and Annotation}
\label{sec:data}

\paragraph{Existing Datasets}
A comprehensive dataset is necessary for evaluation of occlusion boundary detection in dynamic scenes. However, existing datasets are limited in how they only provide ground truth annotation for a single frame from the whole sequence, and don't include information about semantic class labels. This poses a hurdle in the study of the role of the scene structure, and dynamics for occlusion reasoning. Two widely used datasets for occlusion detection in videos are proposed by Stein ~\etal\cite{stein2009occlusion} and Sundberg~\etal\cite{sundberg2011occlusion}. These datasets are limited in their scope as  (1) they provide ground-truth for only a single frame; (2) they are not suitable for the study of the role of the scene layout in occlusion reasoning and were not developed for that purpose. Butler \etal \cite{Butler:ECCV:2012} developed MPI-Sintel flow dataset which contains motion boundaries but does not include the occlusion boundaries in static background. The only dataset with semantic labels, and occlusion boundaries was proposed by Hoiem ~\etal\cite{hoiem2007occl}. They proposed a dataset of 50 images with ground truth annotation of outdoor scenes with occlusion boundaries, surface layout, and depth order. Since this dataset contains only a single image for a scene, it is also not ideal for our study. To overcome this limitation, and we provide a comprehensive dataset for evaluation of our and future research.
% we propose a video dataset with annotated occlusion boundaries of outdoor videos.
%proposed a widely used dataset of 30 image sequences of 20 frames each. Each image sequence has object/occlusion boundary annotated for the center frame only.
%Other widely used dataset for evaluation of occlusions detection is Middlebury dataset []. Middlebury dataset provides ground truth motion estimates for only 19 images sequence of 8 frames and has similar limitations (for our study).
%%% assumption that camera is at a person hieght n horizon 
%%% others are static images, we have moving camera with moving environment
\paragraph{A Video Dataset for Occlusion Reasoning} Our dataset consists of 30 outdoor videos of urban scenes. Some videos were recorded while walking, some while driving, and others were downloaded from YouTube. The videos contain sky, ground, roads, pavements, rivers, buildings, trees, humans, and cars.  To annotate a video, we first over-segment a video into spatio-temporal regions~\cite{MatthiasSegmentation}. Then we group together the spatio-temporal voxels that belong to individual objects, as well as geometric class labels. Geometric classes annotated in our dataset are sky, ground (roads, pavements, grass, rivers),  planer surfaces (buildings and rocks), porous (trees and foliage), and movable objects (humans, cars, and trains). Boundaries between individual objects and geometric classes provide occlusion boundaries. In some cases the segmentation algorithm fails to segment a region due to similarity in color or poor-lighting condition. These boundaries are not annotated in our dataset but such cases are only a small fraction of the whole dataset. The proposed dataset contains 5,042 annotated frames across 30 videos. \Cref{Table:occl_data} provides a comparison of our dataset with existing datasets.
%We selected the videos to provide a mix of these scene examples.
%selected from recently proposed geometric context dataset \cite{Raza2013GCFV}.
%Then we assign these objects to depth ordered layers. We do not assume any fixed number of layers.
%%% make table
\begin{table}%[htb]
\centering
\small
\begin{tabular}{|c|c|c|}\hline
Name & Image/Video & Ground-truth \\\hline
\emph{CMU Geometric Context}~\cite{hoiem2007occl} & Image & 50  \\\hline
\emph{CMU Occlusion}~\cite{stein2007combining} & Video &  30 \\\hline
\emph{BSDS}~\cite{sundberg2011occlusion} & Video & 60  \\\hline
%\emph{Middlebury}~\cite{baker2011database} & Video & 19 \\\hline
\emph{Ours} & Video & 5042 \\\hline
%\emph{mix} & 0.5   \\\hline
\end{tabular}

\caption{Comparison with existing datasets providing ground truth for occlusion boundaries. Our dataset contains 5042 frame across 30 videos with annotations for occlusion boundaries, and geometric class labels.}
\label{Table:occl_data}
\end{table}

==> relatex.tex <==
\section{Related Research}
\label{sec:related}

%%% first write about occlusion detection contribution


%%% video segmentation contribution

%%% layer and depth contribution

%%%% dataset contribution
